Fast and Flexible Inference Framework for Continuum Reverberation Mapping using Simulation-based Inference with Deep Learning

Continuum reverberation mapping (CRM) of active galactic nuclei (AGN) monitors multiwavelength variability signatures to constrain accretion disk structure and supermassive black hole (SMBH) properties. The upcoming Vera Rubin Observatory's Legacy Survey of Space and Time (LSST) will survey tens of millions of AGN over the next decade, with thousands of AGN monitored with almost daily cadence in the deep drilling fields. However, existing CRM methodologies often require long computation time and are not designed to handle such large amount of data. In this paper, we present a fast and flexible inference framework for CRM using simulation-based inference (SBI) with deep learning to estimate SMBH properties from AGN light curves. We use a long-short-term-memory (LSTM) summary network to reduce the high-dimensionality of the light curve data, and then use a neural density estimator to estimate the posterior of SMBH parameters. Using simulated light curves, we find SBI can produce more accurate SMBH parameter estimation with $10^3-10^5$ times speed up in inference efficiency compared to traditional methods. The SBI framework is particularly suitable for wide-field RM surveys as the light curves will have identical observing patterns, which can be incorporated into the SBI simulation. We explore the performance of our SBI model on light curves with irregular-sampled, realistic observing cadence and alternative variability characteristics to demonstrate the flexibility and limitation of the SBI framework.

==> extra.tex <==
%Nonetheless, these CRM campaigns have provided valuable observations to test theoretical accretion disk models. For example, accretion disk profiles typically follow the wavelength-lag relations predicted by the standard \cite{Shakura_Sunyave_1973} accretion disk model. However, while \citep{Homayouni_etal_2019} and \citep{Yu_etal_2020} report accretion disk sizes consistent with standard model, \citep{Jiang_etal_2017} and other intensive CRM programs have found accretion disks are typically 2-3 times larger than prediction \citep{Edelson_etal_2015, Fausnaugh_etal_2016, Jiang_etal_2017}.
%For example, \citep{Jiang_etal_2017} and other intensive CRM programs have found accretion disks are typically 2-3 times larger than the standard \cite{Shakura_Sunyave_1973} accretion disk model \citep{Edelson_etal_2015, Fausnaugh_etal_2016, Jiang_etal_2017}, while \citep{Homayouni_etal_2019} and \citep{Yu_etal_2020} report accretion disk sizes consistent with the standard thin disk. %RM programs with both X-ray and UV/Optical observations also revealed poor correlation between X-ray and UV/Optical variability, suggesting X-ray does not directly drive the UV/Optical light curves \citep{Starkey_etal_2017, Edelson_etal_2017, McHardy_etal_2018, HernandezSantisteban_etal_2020, Cackett_etal_2023}.

\begin{table*}[h]
%\hspace{-2cm}
    \centering
    \begin{tabular}{llrrr}
    \hline\hline
      Name  & \hspace{8.5mm} Network Setup (Output dimensions) & $\sigma$(cos($i$)) & $\sigma$($\log{M}_{\rm BH}$) & $\sigma$($\log{\dot{M}}$) \\
    \hline
    Default SBI & \begin{tabular}[c]{@{}l@{}}No embedding summary network (180x7) \\
                MAF \end{tabular}    
        & 0.10    & 0.33 & 0.23 \\
    \hline
    CNN     & \begin{tabular}[c]{@{}l@{}}CNN (180x7)\\ 
                \hspace{5mm} Conv2d: 6 channels, 5x2 kernels (6x180x7)\\ 
                \hspace{5mm} MaxPool2d: 3x3 kernels (6x60x2)\\ 
                \hspace{5mm} Linear: 16 output features (1x16)\\ 
                MAF \end{tabular} 
        & 0.06 & 0.14 & 0.09 \\
    \hline
    {\bf LSTM (last timestep)}    & \begin{tabular}[c]{@{}l@{}}LSTM (180x7)\\
                \hspace{5mm} LSTM: 64 units (1x64)\\ 
                \hspace{5mm} Linear: 16 output features (1x16)\\     
                MAF \end{tabular}                           
        & {\bf 0.01}   & {\bf 0.08} & {\bf 0.08} \\
    \hline
    LSTM (all timesteps)   & \begin{tabular}[c]{@{}l@{}}LSTM (180x7)\\
                \hspace{5mm} LSTM: 64 units (1x180x64)\\ 
                \hspace{5mm} Linear: 16 output features (1x16)\\     
                MAF \end{tabular}                           
        &  0.01  & 0.09 & 0.08 \\
    \hline\hline
    \end{tabular}
    \caption{Results from alternative SBI configurations.}
    \label{tab:SBIparameters}
\end{table*}   

